Critical Peaks Redefined - $\Phi \sqcup \Psi = \top$

Let a cluster be a term with a number of patterns occurring in it. We give two accounts of clusters, a geometric one as sets of (node and edge) positions, and an inductive one as pairs of terms with gaps (2nd order variables) and pattern-substitutions for the gaps. We show both notions of cluster and the corresponding refinement/coarsening orders on them, to be isomorphic. This equips clusters with a lattice structure which we lift to (parallel/multi) steps to yield an alternative account of the notion of critical peak.

==> cpr-macros-iwc2017.tex <==

% bertram's hack for converse superscripts, adapted from harald
\makeatletter
\def\lubd#1#2#3{%
 \def\next##1##2{%
  \setbox0=\hbox{$##1\vphantom{#3}\@ifempty{#1}{}{_{\vphantom{#1}}}%
   \@ifempty{#2}{}{^{#2}}$}%
  \setbox1=\hbox{$##1\vphantom{#3}\@ifempty{#1}{}{_{#1}}%
   \@ifempty{#2}{}{^{\vphantom{#2}}}$}%
  \setbox2=\vbox{\hbox to\wd0{}\hbox to\wd1{}}%
  {\hskip\wd2\hskip-\wd0\box0\hskip-\wd1\box1{#3}}%
 }%
 \mathpalette\next{}%
}
\def\lud#1#2#3{{\lubd{#1}{#2}{#3}}}
\def\rubd#1#2#3{#3\@ifempty{#1}{}{_{#1}}\@ifempty{#2}{}{^{#2}}}
\def\rubd#1#2#3{{\rubd{#1}{#2}{#3}}}
\makeatother
% ... \lud{subscript}{superscript}{arrow} ... 
% application by super/subscripting, clockwise, based on shape of letters:
% o = 0 (top-right), i = 1 (bottom-right), z = 2 (bottom-left), e = 3 (top-left)
\def\op#1#2{#1^{#2}}
\def\ip#1#2{#1_{#2}}
\def\zp#1#2{\lud{#2}{}{#1}}
\def\ep#1#2{\lud{}{#2}{#1}}

% compose multistep symbol
\catcode`\@=11
\newcommand{\wash}{\mathpalette\mywash}
\newcommand{\mywash}[2]{\setbox0=\hbox{$\m@th#1{#2}$}\wd0=0pt\box0}
\catcode`\@=12
\newcommand{\arsdev}{\mathrel{\wash{\,\,\,\circ}\mathord{\longrightarrow}}}
\newcommand{\arsdevinv}{\mathrel{\wash{\,\,\,\,\circ}\mathord{\longleftarrow}}}

% placeholder alternative to dots
\def\lscore{{\_}}

% for boxing nested subterms
\fboxsep=.4\fboxsep

% greek letters with roman equivalent, for regularity reasons
\def\Alpha{{A}}
\def\Beta{{B}}
\def\Epsilon{{E}}
\def\Zeta{{Z}}
\def\Eta{{H}}
\def\Iota{{I}}
\def\Kappa{{K}}
\def\Mu{{M}}
\def\Nu{{N}}
\def\omicron{o}
\def\Omicron{O}
\def\Rho{{P}}
\def\Tau{{T}}
\def\Chi{{X}}


\def\isdefd{=} % is defined
\def\defdis{=} % defines  

\def\hastype{\mathbin{:}} % has type
\def\hastyp{\hastype} % variant spelling of macro
\def\stypfun{{\to}} % function type
\def\typfun{\binap{\stypfun}}

% different ways for denoting application
\def\relap#1#2#3{#2\mathrel{#1}#3} % infix with relation spacing
\def\binap#1#2#3{#2\mathbin{#1}#3} % infix with binary operation spacing
\def\funap#1#2{#1(#2)} % prefix with parentheses
\def\funsep{,}
\def\funbap#1#2#3{\funap{#1}{#2\funsep#3}} % prefix with two arguments
\def\str#1{\langle#1\rangle} % making a structure
\def\pairsep{{,}}
\def\pair#1#2{(#1\pairsep#2)} % pairing

\def\aset{{A}} % sets
\def\bset{{B}}
\def\cset{{C}}
\def\dset{{D}}
\def\ssetin{{\in}}  % set membership
\def\setin{\binap{\ssetin}}
\def\setstr#1{\{#1\}} % set structure
\def\setabs#1#2{\setstr{#1\mathrel{|}#2}} % set comprehension
\def\sseteq{{=}}
\def\seteq{\relap{\sseteq}}
\def\ssetle{{\subseteq}} % subset
\def\setle{\relap{\ssetle}}
\def\ssetgt{{\supset}} % subset
\def\setgt{\relap{\ssetgt}}
\def\setemp{{\emptyset}} % empty set
\def\ssetlub{{\cup}} % set (non-disjoint) union 
\def\setlub{\binap{\ssetlub}}
\def\ssetLub{\bigcup} % Union
\def\setLub#1#2{\ssetLub_{#1}{#2}}
\def\ssetsum{{\uplus}} % set (disjoint) union/sum
\def\setsum{\binap{\ssetsum}}
\def\ssetdif{{-}} % set difference
\def\setdif{\binap{\ssetdif}}
\def\ssetpow{{\powerset}} % power set
\def\setpow#1{\ssetpow#1}
\def\setpowne#1{\ip{\ssetpow}{\mathit{ne}}#1}
\def\ssetanti{\Arrowvert} % antichain
\def\setanti#1{{\left\ssetanti#1\right\ssetanti}}
\def\ssetglb{{\cap}}
\def\setglb{\binap{\ssetglb}}

\def\srelref{{=}} % reflexive closure
\def\relref#1{\op{#1}{\srelref}}
\def\sreltra{{+}} % transitive closure
\def\reltra#1{\op{#1}{\sreltra}}
\def\sreltre{{\ast}} % reflexive-transitive closure
\def\reltre#1{\op{#1}{\sreltre}}
\def\sreltred{{1}} % transitive reduct
\def\reltred#1{\op{#1}{\sreltred}}

%\def\srelser{\raisebox{-.4ex}{\begin{sideways}$\bigotriangle$\end{sideways}}}
\def\srelser{{\olessthan}} % serial composition
\def\relser{\relap{\srelser}}
\def\srelsco{{\cdot}} % sequential composition
\def\relsco{\binap{\srelsco}}
\def\srellub{{\ssetlub}} % union
\def\rellub{\relap{\srellub}}
\def\srellex{\ip{\times}{\mathsf{lex}}} % lexicographic product
\def\rellex{\binap{\srellex}}
\def\srelle{{\ssetle}}
\def\relle{\relap{\srelle}}

\def\sfuncom{{\circ}}
\def\funcom#1#2{\binap{\sfuncom}{#2}{#1}}

\def\aord{{\succ}}
\def\orda{\relap{\aord}}
\def\ordstr{\pair}
\def\shoa{{H}}
\def\aordhoa{\ip{\aord}{\shoa}}
\def\ordhoaa{\relap{\aordhoa}}
\def\aordhot{\hot{\aord}}
\def\ordhota{\relap{\aordhot}}
\def\aorddwn{{\curlyvee}}
\def\orddwna#1{{\aorddwn#1}}
\def\aorddwnhot{\hot{\aorddwn}}
\def\orddwnhota#1{{\aorddwnhot#1}}
%\def\sorditf{\ip{\snatgt}{\sclsitf}}
\def\sorditf{\snatggt}
\def\orditf{\relap{\sorditf}}
%\def\sorditfref{\ip{\snatge}{\sclsitf}}
\def\sorditfref{\snatgge}
\def\orditfref{\relap{\sorditfref}}

% natural numbers
\def\Nat{\mathbb{N}}
% \def\Pos{\ip{\Nat}{+}} renamed to avoid clash with positions
\def\Natp{\ip{\Nat}{+}}
\def\natzer{{0}}
\def\natone{{1}}
\def\nattwo{{2}}
\def\natthr{{3}}
\def\natfou{{4}}
\def\anat{{n}}
\def\bnat{{m}}
\def\cnat{{k}}
\def\ainat{\ip{\anat}}
\def\binat{\ip{\bnat}}
\def\cinat{\ip{\cnat}}
\def\snatgt{{>}}
\def\natgt{\relap{\snatgt}}
\def\snatlt{{<}}
\def\natlt{\relap{\snatlt}}
\def\snateq{{=}}
\def\nateq{\relap{\snateq}}
\def\snatle{{\leqslant}} 
% VvO changed to slanted version(s) to avoid ambiguity
% on how to interpret >>
% (1) as the strict part of the lex product of \geq with itself
% (2) as the lex product of > with itself
% using geqslant only leaves interpretation (1), as intended
\def\natle{\relap{\snatle}}
\def\snatge{{\geqslant}}
\def\natge{\relap{\snatge}}
\def\snatnle{{\nleqslant}}
\def\natnle{\relap{\snatnle}}
\def\snatnge{{\ngeqslant}}
\def\natnge{\relap{\snatnge}}
\def\snatgge{\raisebox{.06em}{$\lefteqn{\kern.06em\underline{\phantom{\kern.1em>}}}{\gg}$}}
%\def\snatgge{{\kern-.03em{\geq}\kern-.53em{\geq}}} % VvO does not work, because of MnSymbols?
\def\natgge{\relap{\snatgge}}
\def\snatggt{{\gg}}
\def\natggt{\relap{\natggt}}
\def\snatsum{{+}}
\def\natsum{\binap{\snatsum}}
\def\snatSum{{\sum}}
\def\natSum#1#2{\ip{\snatSum}{#1}#2}
\def\natsuc#1{\natsum{#1}{\natone}}
\def\snatdif{{-}}
\def\natdif{\binap{\snatdif}}
\def\natnum{\ainat{\mathsf{com}}} % number of components in interference
\def\natsiz{\ainat{\mathsf{ovl}}} % amount of overlap in interference
\def\snatglb{{\min}}
\def\snatlub{{\max}}

% indices
\def\aidx{{i}}
\def\bidx{{j}}
\def\cidx{{k}}
\def\aidxsuc{\natsuc{\aidx}}

% abstract rewrite systems
\def\aars{{\to}}
\def\arsa{\relap{\aars}}
\def\aiars{\ip{\aars}}
\def\iarsa#1{\relap{\aiars{#1}}}
\def\aarstra{\reltra{\aars}}
\def\arstraa{\relap{\aarstra}}
\def\aiarstra{\ip{\aarstra}}
\def\iarstraa#1{\relap{\aiarstra{#1}}}
\def\aarsinv{{\leftarrow}}
\def\arsinva{\relap{\aarsinv}}
\def\aiarsinv{\zp{\aarsinv}}
\def\iarsinva#1{\relap{\aiarsinv{#1}}}
\def\aarsdev{{\arsdev}}
\def\arsdeva{\relap{\aarsdev}}
\def\aiarsdev{\ip{\aarsdev}}
\def\iarsdeva#1{\relap{\aiarsdev{#1}}}
\def\aarsdevinv{{\arsdevinv}}
%NH a is lacking 
%\def\arsdevinv{\relap{\aarsdevinv}}
\def\arsdevinva{\relap{\aarsdevinv}}
\def\aiarsdevinv{\zp{\aarsdevinv}}
\def\iarsdevinva#1{\relap{\aiarsdevinv{#1}}}
\def\bars{\Blue{\triangleright}}
\def\arsb{\relap{\bars}}
\def\biars{\ip{\bars}}
\def\iarsb#1{\relap{\biars{#1}}}
\def\barsinv{\Blue{\triangleleft}}
\def\arsinvb{\relap{\barsinv}}
\def\biarsinv{\zp{\barsinv}}
\def\iarsinvb#1{\relap{\biarsinv{#1}}}
\def\barsref{\relref{\bars}}
\def\arsrefb{\relap{\barsref}}
\def\biarsref{\ip{\barsref}}
\def\iarsrefb#1{\relap{\biarsref{#1}}}
\def\barsinvref{\relref{\barsinv}}
\def\arsinvrefb{\relap{\barsinvref}}
\def\biarsinvref{\zp{\barsinvref}}
\def\iarsinvrefb#1{\relap{\biarsinvref{#1}}}
\def\cars{\Red{\blacktriangleright}}
\def\arsc{\relap{\cars}}
\def\ciars{\ip{\cars}}
\def\iarsc#1{\relap{\ciars{#1}}}
\def\carsinv{\Red{\blacktriangleleft}}
\def\arsinvc{\relap{\carsinv}}
\def\ciarsinv{\zp{\carsinv}}
\def\iarsinvc#1{\relap{\ciarsinv{#1}}}
\def\carsref{\relref{\cars}}
\def\arsrefc{\relap{\carsref}}
\def\ciarsref{\ip{\carsref}}
\def\iarsrefc#1{\relap{\ciarsref{#1}}}
\def\carsinvref{\relref{\carsinv}}
\def\arsinvrefc{\relap{\carsinvref}}
\def\ciarsinvref{\zp{\carsinvref}}
\def\iarsinvrefc#1{\relap{\ciarsinvref{#1}}}
\def\bcars{{\barsinv\kern-.31em\cars}}
\def\arsbc{\relap{\bcars}}
\def\bciars{\ip{\bcars}}
\def\iarsbc#1{\relap{\bciars{#1}}}
\def\bcarstre{\reltre{\bcars}}
\def\arstrebc{\relap{\bcarstre}}
\def\bciarstre{\ip{\bcarstre}}
\def\iarstrebc#1{\relap{\bciarstre{#1}}}
\def\aarstre{{\twoheadrightarrow}}
\def\arstrea{\relap{\aarstre}}
\def\aiarstre{\ip{\aarstre}}
\def\iarstrea#1{\relap{\aiarstre{#1}}}
\def\sarsle{{\srelle}}
\def\arsle{\relap{\sarsle}}

% objects
\def\aobj{{a}} % objects
\def\bobj{{b}}
\def\cobj{{c}}
\def\dobj{{d}}
\def\aiobj{\ip{\aobj}}
\def\sobjeq{{=}} % equality
\def\objeq{\relap{\sobjeq}}

% steps
\def\astp{{\phi}}
\def\bstp{{\psi}}
\def\cstp{{\chi}}
\def\dstp{{\omega}}
\def\aistp{\ip{\astp}}
\def\bistp{\ip{\bstp}}
\def\cistp{\ip{\cstp}}
\def\aStp{{\Phi}}
\def\bStp{{\Psi}}
\def\cStp{{\Chi}}
\def\aiStp{\ip{\aStp}}
\def\biStp{\ip{\bStp}}
\def\ciStp{\ip{\cStp}}
\def\sstplub{{\sclslub}}
\def\stplub{\binap{\sstplub}}
\def\sstpglb{{\sclsglb}}
\def\stpglb{\binap{\sstpglb}}
\def\sstpGlb{{\sclsGlb}}
\def\stpGlb{\ip{\sstpGlb}}
\def\sstpLub{{\sclsLub}}
\def\stpLub{\ip{\sstpLub}}
\def\sstpsrc{\mathsf{src}}
\def\stpsrc{\funap{\sstpsrc}}
\def\sstptgt{\mathsf{tgt}}
\def\stptgt{\funap{\sstptgt}}
\def\sstpitf{{\sclsitf}} % interference
\def\stpitf{\funbap{\sstpitf}}
\def\sstpsiz{{\sclssiz}} % inner size, amount of overlap
\def\stpsiz{\funbap{\sstpsiz}}
\def\sstpnum{{\sclsnum}} % outer size, number of components
\def\stpnum{\funbap{\sstpnum}}
\def\sstpeq{\sclseq} % equality
\def\stpeq{\relap{\sstpeq}}
\def\sstpneq{\sclsneq} % inequality
\def\stpneq{\relap{\sstpneq}}
\def\stpbot{\clsbot}
\def\sstpin{{\sclsin}} % step in a multistep
\def\stpin{\binap{\sstpin}}
\def\sistpin{\ip{\sstpin}} % indexed by meta-variable
\def\istpin#1{\binap{\sistpin{#1}}}

% symbols
\def\aSym{{\Sigma}} % signature as set of symbols
\def\asig{\aSym} % alternative def as independent entity
\def\asym{{f}}
\def\bsym{{g}}
\def\csym{{h}}
\def\symap{\funap}
\def\bluesymap#1#2{\Blue{#1(}#2\Blue{)}}
\def\syma{\symap{\asym}} % functions symbols
\def\symb{\symap{\bsym}}
\def\symc{\symap{\csym}}
\def\asymzer{{\aobj}} % nullary function symbols
\def\bsymzer{{\bobj}}
\def\csymzer{{\cobj}}
\def\ssymeq{{\sobjeq}} % equality
\def\symeq{\binap{\ssymeq}}

% rules
\def\aRul{{R}}
\def\bRul{{S}}
\def\cRul{{T}}
\def\dRul{{C}}
\def\arul{{\varrho}}
\def\brul{{\theta}}
\def\crul{{\eta}}
\def\rula{\funap{\arul}}
\def\rulb{\funap{\brul}}
\def\rulc{\funap{\crul}}
\def\srulstr{{\to}}
\def\rulstr{\binap{\srulstr}}

% terms
\def\sTrm{\mathit{Ter}}
\def\sMTrm{\mathit{MTer}}
\def\Trm{\funap{\sTrm}}
\def\MTrm{\funap{\sMTrm}}
\def\Trmover#1#2{\Trm{#1,#2}}
\def\TrmOver#1#2#3{\Trm{#1,#2,#3}}
\def\MTrmover#1#2{\MTrm{#1,#2}}
\def\MTrmOver#1#2#3{\MTrm{#1,#2,#3}}
\def\atrm{{t}}
\def\btrm{{s}}
\def\ctrm{{u}}
\def\dtrm{{w}}
\def\etrm{{p}}
\def\ftrm{{q}}
\def\gtrm{{o}}
\def\amtrm{{M}}
\def\bmtrm{{N}}
\def\cmtrm{{L}}
\def\dmtrm{{K}}
\def\emtrm{{J}}
\def\cimtrm{\ip{\cmtrm}}
\def\alhs{{\ell}}
\def\ailhs{\ip{\alhs}}
\def\blhs{{g}}
\def\crhs{{h}}
\def\arhs{{r}}
\def\airhs{\ip{\arhs}}
\def\brhs{{d}}
\def\crhs{{m}}
\def\aitrm{\ip{\atrm}}
\def\bitrm{\ip{\btrm}}
\def\citrm{\ip{\ctrm}}
\def\ditrm{\ip{\dtrm}}
\def\eitrm{\ip{\etrm}}
\def\fitrm{\ip{\ftrm}}
\def\gitrm{\ip{\gtrm}}
\def\aimtrm{\ip{\amtrm}}
\def\bimtrm{\ip{\bmtrm}}
\def\cimtrm{\ip{\cmtrm}}
\def\dimtrm{\ip{\dmtrm}}
\def\eimtrm{\ip{\emtrm}}
\def\strmeq{{=}} % equality
\def\trmeq{\relap{\strmeq}}
\def\strmneq{{\neq}} % inequality
\def\trmneq{\relap{\strmneq}}
\def\strmvar{\mathsf{v}}
\def\trmvar{\ip{\strmvar}}
\def\atrmvar{{x}}
\def\btrmvar{{y}}
\def\ctrmvar{{z}}
\def\dtrmvar{{w}}
\def\etrmvar{{v}}
\def\ftrmvar{{u}}
\def\Trmvar{\mathit{Var}}
\def\FTrmvar{\mathit{Fvar}}
\def\varmvar{\uppercase}
\def\amtrmvar{\varmvar\atrmvar}
\def\bmtrmvar{\varmvar\btrmvar}
\def\cmtrmvar{\varmvar\ctrmvar}
\def\dmtrmvar{\varmvar\dtrmvar}
\def\emtrmvar{\varmvar\etrmvar}
\def\fmtrmvar{\varmvar\ftrmvar}
\def\cimtrmvar{\ip{\cmtrmvar}}
\def\mtrmvara{\funap{\amtrmvar}}
\def\mtrmvarb{\funap{\bmtrmvar}}
\def\mtrmvarc{\funap{\cmtrmvar}}
\def\mtrmvard{\funap{\dmtrmvar}}
\def\mtrmvare{\funap{\emtrmvar}}
\def\mtrmvarf{\funap{\fmtrmvar}}
\def\MTrmvar{\mathit{MVar}}
\def\FMTrmvar{\mathit{FMVar}}
% encompassment symbol as defined and used by Aart in book
\def\trmenc{\relap{\makebox[0pt]{\makebox[9pt][r]{\raise 0.6pt \hbox{$\cdot$}}}{\trianglerighteq}}}
\def\strmenc{\trmenc{}{}}
%\newcommand{\prencompasses}{\mathrel{\makebox[0pt]{\makebox[9pt][r]%
%{\lower 0.5pt \hbox{$\cdot$}}}{\vartriangleright}}}
\def\trmencinv{\relap{\makebox[0pt]{\makebox[9pt][r]{\raise 0.6pt \hbox{$\cdot$}}}{\trianglelefteq}}}
\def\strmencinv{\trmencinv{}{}}
%\newcommand{\prcontain}{\mathrel{\makebox[0pt]{\makebox[12pt][r]%
%{\lower 0.5pt \hbox{$\cdot$}}}{\vartriangleleft}}}
\def\strmint{\mathsf{Int}} % interior of a term VvO : should now be obsolete, replace by trmstd
\def\strmstd{\mathsf{Std}} 
\def\trmint{\funap{\strmint}} % VvO : obsolete as well
\def\trmstd{\funap{\strmstd}} 
\def\strmsiz{{\#}}
\def\trmsiz{\funap{\strmsiz}}
\def\strmlub{{\vee}} % join wrt subsumption
\def\trmlub{\binap{\strmlub}}
\def\strmglb{{\wedge}}
\def\trmglb{\binap{\strmglb}}
\def\strmsub{{\triangleleft}}
\def\trmsub{\relap{\strmsub}}
\def\strmsubeq{{\trianglelefteq}}
\def\trmsubeq{\relap{\strmsubeq}}
\def\strmsup{{\triangleright}}
\def\trmsup{\relap{\strmsup}}
\def\strmsupeq{{\trianglerighteq}}
\def\trmsupeq{\relap{\strmsupeq}}
\def\trmsbmeq{\relap{\makebox[0pt]{\makebox[15pt][r]{\raise 0.9pt \hbox{$\cdot$}}}{\leq}}}
\def\strmsbmeq{\trmsbmeq{}{}}
\def\trmspmeq{\relap{\makebox[0pt]{\makebox[9pt][r]{\raise 0.9pt \hbox{$\cdot$}}}{\geq}}}
\def\strmspmeq{\trmspmeq{}{}}





% algebras
\def\setalg{\mathcal}
\def\aalg{\setalg{\aset}}
\def\balg{\setalg{\bset}}
\def\salgsum{\mathsf{Sum}}
\def\algsum{\algap{\salgsum}}
\def\salgsiz{\mathsf{Size}}
\def\algsiz{\algap{\salgsiz}}
\def\salgshi{\mathsf{Shift}}
\def\algshi{\algap{\salgshi}}
\def\salgtre{\mathsf{Tree}}
\def\algtre{\algap{\salgtre}}
\def\sfuncut{\text{\Rightscissors}}
\def\funcut{\funbap{\sfuncut}}
%\def\algap#1#2{{\op{\llbracket#2\rrbracket}{#1}}} % VvO leads to too many brackets
\def\algap#1#2{\op{#2}{#1}}
\def\alga{\algap{\aalg}}
\def\algb{\algap{\balg}}
\def\apalg{{\Uparrow}}
\def\sfunsuc{\mathsf{Succ}}
\def\palga{\funap{\apalg}}

% position (algebras)
\def\sPos{\mathcal{{P}\mathit{os}}}
\def\Pos{\funap{\sPos}}
\def\apos{p}
\def\bpos{q}
\def\cpos{r}
\def\aPos{P}
\def\bPos{Q}
\def\cPos{R}
\def\aiPos{\ip{\aPos}}
\def\biPos{\ip{\bPos}}
\def\ciPos{\ip{\cPos}}
\def\spossco{{\cdot}}
\def\possco#1#2{#1\spossco#2}
\def\amPos{{\Pi}}
\def\bmPos{{\Phi}}
\def\posedge{{\mbox{--}}}
\def\vtxpos#1{\mathring{#1}}
\def\edgpos#1{\bar{#1}}
\def\posemp{\varepsilon}
\def\aedgidx{\edgpos{\imath}}
\def\bedgidx{\edgpos{\jmath}}
\def\avtxidx{\vtxpos{\imath}}
\def\bvtxidx{\vtxpos{\jmath}}
\def\posone{1}
\def\postwo{2}
\def\posthr{3}
\def\aimPos{\ip{\amPos}}
\def\bimPos{\ip{\bmPos}}
\def\cimPos{\ip{\cmPos}}


% contexts
\def\actx{C}
\def\bctx{D}
\def\cctx{E}
\def\ctxap#1#2{#1[#2]}
\def\ctxa{\ctxap{\actx}}
\def\ctxb{\ctxap{\bctx}}
\def\ctxc{\ctxap{\cctx}}
\def\ctxemp{{\Box}}

% patterns (VvO: used?)
%\def\apat{{p}}
%\def\bpat{{q}}
%\def\cpat{{r}}
\def\apat{\alhs}
\def\bpat{\blhs}
\def\cpat{\clhs}

% clusters
\def\acls{{\varsigma}} 
\def\bcls{{\zeta}}
\def\ccls{{\xi}}
\def\aicls{\ip{\acls}}
\def\bicls{\ip{\bcls}}
\def\cicls{\ip{\ccls}}
\def\aCls{\mathcal{E}} % sets of clusters
\def\bCls{\mathcal{F}}
\def\cCls{\mathcal{G}}
\def\clsstr#1#2{\pair{#1}{#2}}
\def\clsbox#1{\fbox{\vphantom{$($}$#1$}}
\def\clsboxa#1{\funap{\clsbox{#1}}}
\def\sclsle{{\sqsubseteq}} % cluster refinement
\def\clsle{\relap{\sclsle}}
\def\sclslt{{\sqsubset}} % strict
\def\clslt{\relap{\sclslt}}
\def\sclsge{{\sqsupseteq}} % cluster refinement
\def\clsge{\relap{\sclsge}}
\def\sclsgt{{\sqsupset}} % strict
\def\clsgt{\relap{\sclsgt}}
\def\sclsletred{\reltred{\sclsle}} % transitive reduct
\def\clsletred{\relap{\sclsletred}}
\def\sclslttred{\reltred{\sclslt}} % transitive reduct
\def\clslttred{\relap{\sclslttred}}
\def\sclslub{{\sqcup}}
\def\clslub{\binap{\sclslub}}
\def\sclsglb{{\sqcap}}
\def\clsglb{\binap{\sclsglb}}
\def\sclsGlb{{\bigsqcap}}
\def\clsGlb{\ip{\sclsGlb}}
\def\sclsLub{{\bigsqcup}}
\def\clsLub{\ip{\sclsLub}}
%\def\sclssiz{{\fbox{\#}}}
\def\sclsin{{\ssetin}}
\def\clsin{\binap{\sclsin}}
\def\sclssiz{\ip{\strmsiz}{\natone}}
\def\clssiz{\funap{\sclssiz}}
%\def\sclsnum{{\#}}
\def\sclsnum{\ip{\strmsiz}{\natzer}}
\def\clsnum{\funap{\sclsnum}}
\def\sclsitf{\mathfrak{I}}
\def\clsitf{\funbap{\sclsitf}}
\def\clsbot{{\bot}} % bottom of cluster lattice
\def\iclsbot{\ip{\clsbot}}
\def\clstop{{\top}} % top of cluster lattice
\def\iclstop{\ip{\clstop}}
\def\sclseq{{\strmeq}} % equality of clusters
\def\clseq{\relap{\sclseq}}
\def\sclsneq{{\strmneq}} % inequality
\def\clsneq{\relap{\sclsneq}}
\def\sclsovl{\op{\sclsovlequ}{\natone}} % has overlap with
\def\siclsovl{\ip{\sclsovl}}
\def\clsovl{\relap{\sclsovl}}
\def\iclsovl#1{\relap{\siclsovl{#1}}}
\def\sclsovlequ{{\bumpeq}} % equivalence closure of has overlap with
\def\clsovlequ{\relap{\sclsovlequ}}
\def\siclsovlequ{\ip{\sclsovlequ}}
\def\iclsovlequ#1{\relap{\siclsovlequ{#1}}}

% term rewrite systems
\def\Rultrs#1{\mathcal{#1}}
\def\atrs{\Rultrs{\aRul}}
\def\btrs{\Rultrs{\bRul}}
\def\ctrs{\Rultrs{\cRul}}
\def\dtrs{\Rultrs{\dRul}}
\def\trsstr#1#2{\pair{#1}{#2}}
\def\strsdif{\ssetdif}
\def\trsdif{\relap{\strsdif}}
\def\strslub{\ssetlub}
\def\trslub{\binap{\strslub}}
\def\strsle{\ssetle}
\def\trsle{\relap{\strsle}}

% substitutions
\def\subap#1#2{\op{#2}{#1}}
\def\substr#1#2{[#1\mathbin{{:}{=}}#2]}
\def\substra#1#2#3{\subap{\substr{#1}{#2}}{#3}}
\def\asub{{\sigma}}
\def\bsub{{\tau}}
\def\csub{{\mu}}
\def\dsub{{\nu}}
\def\suba{\subap{\asub}}
\def\subb{\subap{\bsub}}
\def\subc{\subap{\csub}}
\def\aisub{\ip{\asub}}
\def\msubap#1#2{\subap{#1}{#2}}
\def\msubstr#1#2{\llbracket#1\mathbin{{:}{=}}#2\rrbracket}
\def\msubstra#1#2#3{\msubap{\msubstr{#1}{#2}}{#3}}
\def\amsub{{\alpha}} % metavar-substitution
\def\bmsub{{\beta}}
\def\cmsub{{\gamma}}
\def\dmsub{{\delta}}
\def\emsub{{\epsilon}}
\def\aimsub{\ip{\amsub}} % indexed
\def\bimsub{\ip{\bmsub}}
\def\cimsub{\ip{\cmsub}}
\def\dimsub{\ip{\dmsub}}
\def\eimsub{\ip{\emsub}}
\def\msuba{\msubap{\amsub}} % metasubs-application
\def\msubb{\msubap{\bmsub}}
\def\msubc{\msubap{\cmsub}}
\def\msubd{\msubap{\dmsub}}
\def\msube{\msubap{\emsub}}
\def\imsuba#1{\msubap{\aimsub{#1}}} % indexed
\def\imsubb#1{\msubap{\bimsub{#1}}} % indexed
\def\imsubc#1{\msubap{\cimsub{#1}}} % indexed
\def\imsubd#1{\msubap{\dimsub{#1}}} % indexed
\def\imsube#1{\msubap{\eimsub{#1}}} % indexed
\def\ssubeq{{\strmeq}}
\def\subeq{\relap{\ssubeq}}
\def\ssubcom{{\sfuncom}}
\def\subcom#1#2{\binap{\ssubcom}{#2}{#1}}
\def\subemp{{\setemp}} % the empty substitution
\def\subempa{\subap{\subemp}}
\def\ssublub{{\ssetlub}}
\def\sublub{\binap{\ssublub}}

% labels
\def\Lab#1{\mathcal{#1}}
\def\aLab{\Lab{L}}
\def\aLabhot{\hot{\aLab}}
\def\Laba{\funap{\Lab{L}}}
\def\Labhota{\funap{\aLabhot}}
\def\alab{{\ell}}
\def\blab{{\kappa}}
\def\clab{{\mu}}
\def\dlab{{\nu}}
\def\slabeq{{=}}
\def\labeq{\relap{\slabeq}}

%\def\shot{\mathsf{hot}}
\def\hot#1{\mathring{#1}}

\newcommand{\prsymbol}{\shortmid\!\!\!\shortmid}
\newcommand{\arspr}{\mathrel{\wash{\,\,\,\,\prsymbol}\mathord{\longrightarrow}}}
\newcommand{\arsprinv}{\mathrel{\wash{\,\,\,\prsymbol}\mathord{\longleftarrow}}}
\def\aarspr{{\arspr}}
\def\arspra{\relap{\aarspr}}
\def\aiarspr{\ip{\aarspr}}
\def\iarspra#1{\relap{\aiarspr{#1}}}
\def\aarsprinv{{\arsprinv}}
\def\arsprinva{\relap{\aarsprinv}}
\def\aiarsprinv{\zp{\aarsprinv}}
\def\iarsprinva#1{\relap{\aiarsprinv{#1}}}

\def\asymone{\asym}
\def\bsymone{\bsym}
\def\csymone{\csym}
\def\vposemp{\vtxpos{\posemp}}
\def\eposemp{\edgpos{\posemp}}
\def\vposone{\vtxpos{\posone}}
\def\eposone{\edgpos{\posone}}
\def\vpostwo{\vtxpos{\postwo}}
\def\epostwo{\edgpos{\postwo}}
\def\ssetge{{\supseteq}}
\def\setge{\relap{\ssetge}}


